Guiding Word Equation Solving using Graph Neural Networks (Extended Technical Report)

This paper proposes a Graph Neural Network-guided algorithm for solving word equations, based on the well-known Nielsen transformation for splitting equations. The algorithm iteratively rewrites the first terms of each side of an equation, giving rise to a tree-like search space. The choice of path at each split point of the tree significantly impacts solving time, motivating the use of Graph Neural Networks (GNNs) for efficient split decision-making. Split decisions are encoded as multi-classification tasks, and five graph representations of word equations are introduced to encode their structural information for GNNs. The algorithm is implemented as a solver named DragonLi. Experiments are conducted on artificial and real-world benchmarks. The algorithm performs particularly well on satisfiable problems. For single word \mbox{equations}, DragonLi can solve significantly more problems than well-established string solvers. For the conjunction of multiple word equations, DragonLi is competitive with state-of-the-art string solvers.

==> algorithms/draw-graph-old.tex <==
\begin{algorithm}
	\caption{Construct word equation graph}
	\label{algorithm:draw-one-side}
		\textbf{Input: $w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l}= w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r}$}, graphType
		
		\textbf{Initialize: } $G=(V,E,V_{\text{T}},V_{\text{Var}}),V,E,V_{\text{T}},V_{\text{Var}}=\emptyset$
		
		$V=\{v_{=}\}$,  $v_{=}$ is the equal sign node
		
		\For{$t$ in $list(w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l}) \cup list(w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r})$}
		{
		$V = V \cup \{t\}$
		
		$\textbf{if}$ $t \in \Psi $ $\textbf{then}$  $V_{\text{T}}=V_{\text{T}} \cup \{t\}$
		
		$\textbf{if}$ $t \in \Gamma$ $\textbf{then}$ $V_{\text{Var}}=V_{\text{Var}} \cup \{t\}$
		
		\Call{DrawOneSide}{$list(w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l})$,graphType}
		\Call{DrawOneSide}{$list(w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r})$,graphType}
		}
	
	\textbf{Function} \Call{DrawOneSide}{termList,graphType}
	
	 currentNode=$v_{=}$
	 
	\While{termList $\neq \emptyset$}{
	 pop a term $t$ from termList
	 
	 $E = E\cup \{(\text{curentNode},t)\}$
	 
	 \textbf{if} graphType $==$ Graph 2 $\wedge$ $t\neq \#$ \textbf{then} $E = E\cup \{(t,v_{=})\}$
	 
	 \If{graphType in (Graph 3, Graph 5) $\wedge$ $t\in \Gamma$}
	 {$E = E\cup \{(t,v_{t})\}$, where $v_{t}=t \wedge v_{t} \in V_{\text{Var}} \wedge v_{t}\notin V$ }
	 
	 \If{graphType in (Graph 4, Graph 5) $\wedge$ $t\in \Psi$}
	 { $E = E\cup \{(t,v_{t}$, where $v_{t}=t \wedge v_{t} \in V_{\text{T}} \wedge v_{t}\notin V$ }
	 

		currentNode = $t$
	}
\end{algorithm}

==> algorithms/draw-graph.tex <==
\begin{algorithm}
	\SetAlgorithmName{Algorithm}{}{}
	\caption{BuildGraph}
	\label{algorithm:draw-graphs}

	\KwIn{
		A conjuncted word equation $\phi$ of the form $w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l} = w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r}$, an int representing the graphType.
	}
	\KwOut{A graph representation of $\phi$ according to graphType}

		$G \leftarrow (V,E,V_{\text{T}},V_{\text{Var}})$\\
        $V,E,V_{\text{T}},V_{\text{Var}} \leftarrow \emptyset$
		
		$V=\{v_{=}\}$,  $v_{=}$ is the equal sign node
		
		\For{$t$ in $list(w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l}) \cup list(w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r})$}
		{
		$V = V \cup \{t\}$
		
		$\textbf{if}$ $t \in \Psi $ $\textbf{then}$  $V_{\text{T}}=V_{\text{T}} \cup \{t\}$
		
		$\textbf{if}$ $t \in \Gamma$ $\textbf{then}$ $V_{\text{Var}}=V_{\text{Var}} \cup \{t\}$
		
		\Call{BuildOneSide}{$list(w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l})$,graphType}
		\Call{BuildOneSide}{$list(w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r})$,graphType}
		}
\end{algorithm}

==> algorithms/draw-one-side.tex <==
\begin{algorithm}
	\caption{Construct word equation graph}
	\label{algorithm:draw-one-side}
		\textbf{Input: $w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l}= w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r}$}, graphType
		
		\textbf{Initialize: } $G=(V,E,V_{\text{T}},V_{\text{Var}}),V,E,V_{\text{T}},V_{\text{Var}}=\emptyset$
		
		$V=\{v_{=}\}$,  $v_{=}$ is the equal sign node
		
		\For{$t$ in $list(w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l}) \cup list(w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r})$}
		{
		$V = V \cup \{t\}$
		
		$\textbf{if}$ $t \in \Psi $ $\textbf{then}$  $V_{\text{T}}=V_{\text{T}} \cup \{t\}$
		
		$\textbf{if}$ $t \in \Gamma$ $\textbf{then}$ $V_{\text{Var}}=V_{\text{Var}} \cup \{t\}$
		
		\Call{DrawOneSide}{$list(w_{1}^{l}\# w_{2}^{l} \# ... \# w_{n}^{l})$,graphType}
		\Call{DrawOneSide}{$list(w_{1}^{r}\# w_{2}^{r} \# ... \# w_{n}^{r})$,graphType}
		}
	
	\textbf{Function} \Call{DrawOneSide}{termList,graphType}
	
	 currentNode=$v_{=}$
	 
	\While{termList $\neq \emptyset$}{
	 pop a term $t$ from termList
	 
	 $E = E\cup \{(\text{curentNode},t)\}$
	 
	 \textbf{if} graphType $==$ Graph 2 $\wedge$ $t\neq \#$ \textbf{then} $E = E\cup \{(t,v_{=})\}$
	 
	 \If{graphType in (Graph 3, Graph 5) $\wedge$ $t\in \Gamma$}
	 {$E = E\cup \{(t,v_{t})\}$, where $v_{t}=t \wedge v_{t} \in V_{\text{Var}} \wedge v_{t}\notin V$ }
	 
	 \If{graphType in (Graph 4, Graph 5) $\wedge$ $t\in \Psi$}
	 { $E = E\cup \{(t,v_{t}$, where $v_{t}=t \wedge v_{t} \in V_{\text{T}} \wedge v_{t}\notin V$ }
	 

		currentNode = $t$
	}
\end{algorithm}

==> algorithms/split-algorithm.tex <==

\begin{algorithm}[tbhp]
	\SetAlgorithmName{Algorithm}{}{}
	\caption{Solve a conjunction of word equations $\phi$}
	\label{algorithm:SolveEqs}
	\KwIn{
		A conjuncted word equation $\phi$ of the form $\bigwedge w_{i}^{l} = w_{i}^{r}$ ($0 \leq i \leq n)$, a backtrack strategy ($BT1,BT2, \text{or } BT3$), a set of initial values for global variable $l$ ($l_{BT2}, l_{BT2}^{step}, l_{BT3}$), a set of terminal symbols $\Psi$, a set of variables $\Gamma$.
	}
	\KwOut{\SAT,\UNSAT, or \UNKNOWN of $\phi$}
	
	
	\textbf{Global variable}: $l=\infty$
	
	\Begin{
		\If{BT1}{
			res=\Call{solveEqs}{$\phi$,0,$\Psi$,$\Gamma$}
		}
		\If{BT2}{
			$l=l_{BT2}$
			
			res=\Call{solveEqs}{$\phi$,0,$\Psi$,$\Gamma$}
		}
		\If{BT3}{			
			$l=l_{BT3}$
			
			\While{True}{
				res=\Call{solveEqs}{$\phi$,0,$\Psi$,$\Gamma$}
				
				\If{res $\neq$ UNKNOWN}{
					break
				}
				$l=l+1$
			}	
		}
		
		\Return res
		
		
		
		
	}
	
	\textbf{Function} \Call{SolveEqs}{$\phi$,$currentDepth$,$\Psi$,$\Gamma$}
	
	\If{$currentDepth \geq l$}{
		%\If{BT1}{pass}
		\If{BT2}{
			$l=l+l_{BT2}^{step}$
			
			\Return{\UNKNOWN}
		}	
		\If{BT3}{
			\Return{\UNKNOWN}
		}
		
	}
	
	%	\If{BT1}{pass}
	%	\If{BT2}{
		%		\If{$currentDepth\geq l_{BT2}$}{
			%			
			%			$l_{BT2}=l_{BT2}+l_{BT2}^{step}$
			%			
			%			\Return UNKNOWN
			%		}
		%	}
	%	\If{BT3}{
		%		\If{$currentDepth\geq l_{BT3}$}{
			%			\Return UNKNOWN
			%		}
		%	}
	
	
	branches=\Call{ApplyRules}{$\phi$,$\Psi$,$\Gamma$}
	
	branches=\Call{orderBranches}{branches}
	
	unknownFlag=0
	
	\For{child $\leftarrow$ branches}{
		res=\Call{SolveEqs}{$child$,$currentDepth+1$,$\Psi$,$\Gamma$}
		
		\If{res==SAT}{
			\Return SAT
		}
		\If{res==UNKNOWN}{
			unknonFlag=1
		}
		
	}
	\eIf{unknownFlag==1}{\Return UNNOWN}{\Return UNSAT}
	
	
\end{algorithm}



==> tables/deduction-tree.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
{
	\tiny
\begin{table}[]
	\begin{tabular}{ccccccccccccccccccccccccc}
		\multirow{2}{*}{$R_{8}$} & \multicolumn{24}{c}{$AbB=bAAC$} \\ \cline{2-25} 
		&  & \multicolumn{12}{c}{[$A \mapsto \epsilon$]} & \multicolumn{1}{c|}{} &  &  & \multicolumn{8}{c}{[$A \mapsto bA'$]} \\
		& \multirow{2}{*}{$R_{10}$} & \multicolumn{12}{c}{$B=C$} & \multicolumn{1}{c|}{} &  & \multirow{2}{*}{$R_{8}$} & \multicolumn{8}{c}{$A'bB=bA'bA'C$} \\ \cline{3-14} \cline{18-25} 
		&  &  & [$B \mapsto \epsilon$] & \multicolumn{1}{c|}{} &  & [$C \mapsto \epsilon$] & \multicolumn{1}{c|}{} &  & [$B \mapsto CB'$] & \multicolumn{1}{c|}{} &  & [$C \mapsto BC'$] &  &  &  &  &  & \multicolumn{2}{c}{[$A' \mapsto \epsilon]$} & \multicolumn{1}{c|}{} &  &  & \multicolumn{2}{c}{[$A' \mapsto bA''$]} \\
		&  & \multirow{2}{*}{$R_{3}$} & $\epsilon=C$ & \multicolumn{1}{c|}{} & \multirow{2}{*}{$R_{3}$} & $B=\epsilon$ & \multicolumn{1}{c|}{} & \multirow{2}{*}{$R_{3}$} & $B'=\epsilon$ & \multicolumn{1}{c|}{} & \multirow{2}{*}{$R_{3}$} & $\epsilon=C'$ &  &  &  &  & \multirow{2}{*}{$R_{8}$} & \multicolumn{2}{c}{$B=bC$} & \multicolumn{1}{c|}{} &  & \multirow{2}{*}{$R_{8}$} & \multicolumn{2}{c}{$A''bB=bA''bA''C$} \\ \cline{4-4} \cline{7-7} \cline{10-10} \cline{13-13} \cline{19-20} \cline{24-25} 
		&  &  & SAT &  &  & SAT &  &  & SAT &  &  & SAT &  &  &  &  &  & \multicolumn{1}{c|}{[$B\mapsto \epsilon$]} & [$B\mapsto bB'$] &  &  &  & \multicolumn{1}{c|}{[$A''\mapsto \epsilon$]} & [$A'' \mapsto bA'''$] \\
		&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \multicolumn{1}{c|}{UNSAT} & ... &  &  &  & \multicolumn{1}{c|}{...} & ...
	\end{tabular}
\end{table}
}

